From Information Theory Puzzles in Deletion Channels to Deniability in Quantum Cryptography

From the output produced by a memoryless deletion channel with a uniformly random input of known length $n$, one obtains a posterior distribution on the channel input. The difference between the Shannon entropy of this distribution and that of the uniform prior measures the amount of information about the channel input which is conveyed by the output of length $m$. We first conjecture on the basis of experimental data that the entropy of the posterior is minimized by the constant strings $\texttt{000}\ldots$, $\texttt{111}\ldots$ and maximized by the alternating strings $\texttt{0101}\ldots$, $\texttt{1010}\ldots$. We present related combinatorial theorems involving binary (sub/super)-sequences and prove the minimal entropy conjecture for single and double deletions using clustering techniques. We then prove the minimization conjecture in the asymptotic limit using results from hidden word statistics by showing how the analytic-combinatorial methods of Flajolet, Szpankowski and Vall\'ee, relying on generating functions, can be applied to resolve the case of fixed output length and $n\rightarrow\infty$. Next, we revisit the notion of deniability in quantum key exchange (QKE). We introduce and formalize the notion of coercer-deniable QKE. We then establish a connection between covert communication and deniability to propose DC-QKE, a simple and provably secure construction for coercer-deniable QKE. We relate deniability to fundamental concepts in quantum information theory and suggest a generic approach based on entanglement distillation for achieving information-theoretic deniability, followed by an analysis of other closely related results such as the relation between the impossibility of unconditionally secure quantum bit commitment and deniability. Finally, we present an efficient coercion-resistant and quantum-secure voting scheme, based on fully homomorphic encryption.

==> preamble/header.tex <==
\makeatletter
\newcommand\thickhrulefill{\leavevmode \leaders \hrule height 1ex \hfill \kern \z@}
\setlength\midchapskip{10pt}
\makechapterstyle{VZ14}{
\renewcommand\chapternamenum{}
\renewcommand\printchaptername{}
\renewcommand\chapnamefont{\Large\scshape}
\renewcommand\printchapternum{%
\chapnamefont\null\thickhrulefill\quad
\@chapapp\space\thechapter\quad\thickhrulefill}
\renewcommand\printchapternonum{%
\par\thickhrulefill\par\vskip\midchapskip
\hrule\vskip\midchapskip
}
\renewcommand\chaptitlefont{\Huge\scshape\centering}
\renewcommand\afterchapternum{%
\par\nobreak\vskip\midchapskip\hrule\vskip\midchapskip}
\renewcommand\afterchaptertitle{%
\par\vskip\midchapskip\hrule\nobreak\vskip\afterchapskip}
}
\makeatother
\chapterstyle{VZ14}
% ***** End memoir chapter title styling

% ***** Start mini chapter TOC code
\newcommand{\minichaptocenabled}{1}

\newcommand{\printminichaptoc}[1]{%
\ifnum0=#1\relax

\else
	\startcontents[chapters]
	\Mprintcontents
\fi
}

\newcommand{\stopminichaptoc}[1]{%
\ifnum0=#1\relax

\else
	\stopcontents[chapters]
\fi
}

% \usepackage{minitoc} %For mini TOC in each chapter (does not play well with the memoir class)
% \usepackage{shorttoc}
\usepackage{titletoc} %For mini TOC in each chapter

\newcommand\partialtocname{Contents}
\newcommand\ToCrule{\noindent\rule[5pt]{\textwidth}{1.3pt}}
\newcommand\ToCtitle{{\small\bfseries\partialtocname}\vskip2pt\ToCrule}
\makeatletter
\newcommand\Mprintcontents{%
  \ToCtitle
  {\footnotesize\ttl@printlist[chapters]{toc}{}{0}{\setcounter{tocdepth}{2}}\par\nobreak
  \ToCrule}}
\makeatother
% ***** End mini chapter TOC code

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lmodern} % Use to remove the report stylesheet's default restrictions on font size
% \usepackage{kpfonts}
% \usepackage{tgpagella}
\usepackage[british]{babel}
\usepackage{csquotes}
% \usepackage[final,activate=true,protrusion=true,kerning=true]{microtype}
\usepackage{zi4}
\usepackage{booktabs}
\usepackage{graphicx}
\graphicspath{ {res/} }

\newcommand{\printtitle}{From Information Theory Puzzles in Deletion Channels to Deniability in Quantum Cryptography}
\newcommand{\prettyprinttitle}{From Information Theory Puzzles in Deletion Channels to \\\vspace{.4em} Deniability in Quantum Cryptography}
\newcommand{\printshorttitle}{From Puzzles in Deletion Channels to Deniability in Quantum Cryptography}
\newcommand{\printauthor}{Arash Atashpendar}

\let\footruleskip\undefined %undefine footruleskip
\usepackage{fancyhdr}
\setlength{\headheight}{21pt}
\pagestyle{fancy}
\fancyhf{}
\lhead{\footnotesize\scshape\nouppercase{\leftmark}}
\rfoot{\footnotesize\thepage}
\lfoot{\footnotesize\scshape\nouppercase{\rightmark}}

\usepackage[a4paper,margin=0.8in]{geometry}
% \usepackage[a4paper]{geometry}
% \usepackage[a4paper,width=150mm,top=25mm,bottom=25mm]{geometry}

%\usepackage{setspace}
%\singlespacing

\usepackage{authblk}

% \usepackage{etex}

\usepackage{graphicx}
\usepackage{tikz}
\usepackage{xcolor}

\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathtools}
%\usepackage{euler}
\usepackage{physics}
\usepackage{algorithm}
\usepackage{algorithmic}
%\usepackage{algorithmicx}
%\usepackage[noend]{algpseudocode}
\usepackage{xfrac}
\usepackage[pdfpagelabels=true]{hyperref}
\usepackage{cleveref}
% \usepackage{varioref}
% \usepackage{url}
%\usepackage{cite}

\hypersetup{
	linktoc = page,
	pdfpagemode = UseNone,
	colorlinks,
	linkcolor={red!50!black},
	citecolor={blue!50!black},
	urlcolor={blue!80!black}
}

% \usepackage[citestyle=numeric,style=numeric,maxnames=10]{biblatex}
% \usepackage[backend=biber,style=ieee,citestyle=numeric,maxnames=10]{biblatex}
% \addbibresource{references.bib}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand*{\bad}[1]{{\textbf{\color{red!50!black}#1}}}
\newcommand*{\E}{\mathbb{E}}
\newcommand*{\good}[1]{{\underline{\color{green!50!black}#1}}}

\newcommand\hlight[1]{\tikz[overlay, remember picture,baseline=-\the\dimexpr\fontdimen22\textfont2\relax]\node[rectangle,fill=gray!50,rounded corners,fill opacity = 0.2,draw,thick,text opacity =1] {$#1$};}

\usepackage{mdframed}
\newcommand{\todo}[1]{ \begin{mdframed}[backgroundcolor=orange!50] #1 \end{mdframed} }

\newcommand{\csquote}[1]{``#1''}

\newcommand{\PP}{\mathbb{P}}
\newcommand{\bigO}[1]{\mathcal{O}(#1)}
\newcommand{\f}[1]{\mathcal{F}_{#1}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\adv}{E}
\newcommand{\view}[1]{\mathrm{View}_{#1}}
\newcommand{\ppt}{\mathrm{PPT}}
\newcommand{\qpt}{\mathrm{QPT}}
\newcommand{\dist}{\mathsf{D}}
\newcommand{\negl}[1]{\mathrm{negl}(#1)}
\newcommand{\prob}[1]{\mathrm{Pr}[#1]}
\newcommand{\sample}{{\leftarrow}\vcenter{\hbox{\tiny\rmfamily\upshape\$}}}
\newcommand{\kgen}{\mathrm{KGen}}
\newcommand{\sk}{\mathrm{sk}}
\newcommand{\pk}{\mathrm{pk}}
\newcommand{\covpi}[1]{\Pi^{cov}_{#1}}

\newcommand{\enc}[2]{E_{#2}(#1)}
\newcommand{\encTerm}[2]{\{{#1}\}_{#2}}
\newcommand{\bb}{\mathfrak{BB}}
\newcommand{\mc}[1]{\mathcal{#1}}


\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}{Conjecture}[theorem]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[theorem]

\theoremstyle{remark}
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]

